On properties of Parisi measures

We investigate the structure of Parisi measures, the functional order parameters of mixed p-spin models in mean field spin glasses. In the absence of external field, we prove that a Parisi measure satisfies the following properties. First, at all temperatures, the support of any Parisi measure contains the origin. If it contains an open interval, then the measure has a smooth density on this interval. Next, we give a criterion on temperature parameters for which a Parisi measure is neither Replica Symmetric nor One Replica Symmetry Breaking. Finally, we show that in the Sherrington-Kirkpatrick model, slightly above the critical temperature, the largest number in the support of a Parisi measure is a jump discontinuity. An analogue of these results is discussed in the spherical mixed p-spin models. As a tool to establish these facts and of independent interest, we study functionals of the associated Parisi PDEs and derive regularity properties of their solutions.

==> invlat.tex <==


%These are definitions for the preamble of TEX files

%\loadmsbm
%that may be needed for \Bbb (``blackboard bold, Bourbaki'') characters
%\UseAMSsymbols
%
%
%\magnification = \magstep1
\font\tencmmib=cmmib10 \skewchar\tencmmib '60
\newfam\cmmibfam
\textfont\cmmibfam=\tencmmib
\def\Ph{\mathchar'4010}
\def\Ps{\mathchar'4011}
\font\tensmc=cmcsc10
\def\smc{\tensmc}
\def\srm{\sevenrm }
%\font\teneufm=EUFM10
%\font\eighteufm=EUFM10 scaled 800
%\def\Fff#1{\hbox{\teneufm#1}}
%\def\Ffff#1{\hbox{\eighteufm#1}}
\font\tenmsb=msbm10
\font\eightmsb=msbm10 scaled 800
\def\Bbb#1{\hbox{\tenmsb#1}}
\def\Bbbb#1{\hbox{\eightmsb#1}}
%\font\bb=msbm10
%\def{\hbox{\bb N}}
%\def\RR{\hbox{\bb R}}
%\def \NN {{I\kern-.3em N}}
%\def \RR {{I\kern-.3em R}}
\def\bbox{\quad\hbox{\vrule \vbox{\hrule \vskip2pt \hbox{\hskip2pt
\vbox{\hsize=1pt}\hskip2pt} \vskip2pt\hrule}\vrule}}
\def\lessim{\ \lower4pt\hbox{$
\buildrel{\displaystyle <}\over\sim$}\ }
\def\gessim{\ \lower4pt\hbox{$\buildrel{\displaystyle >}
\over\sim$}\ }
\def\n{\noindent}
%\def\P{{\rm P}}
%\def\E{{\rm E}}
%\def\LL{{\cal L}}
\def\n{\noindent}
%\parskip=0.03truein
%\hfuzz=0.2truein
%
%\scriptfont4 = \sevensy
%\scriptscriptfont4 = \fivesy
%\font \gross=cmbx10 scaled \magstep2
%\font \mittel=cmbx10 scaled \magstep0  
%\font \outline=ocrb10f scaled \magstep1 
%\pageno = 1
\def\AA{{\cal A} }
\def\AAA{{\bf A} }
\def\Aap{(A,\AA ,P)}
\def\alf{\alpha}
\def\anorm{\|^.\|}
\def\AP{\it Ann. Probab. \bf}
\def\bbe{\vskip .15pc\hangindent=.5pc\hangafter=1}
\def\BB{{\cal B} }
\def\bxt{\boxtimes}
\def\CC{{\cal C} }
\def\claw{\Rightarrow}
\def\cntr{\centerline}
\def\cosph{\cos\phi}
\def\costh{\cos\theta}
\def\DAN{Dokladi AN Ukr.SSR}
\def\DD{{\cal D} }
\def\dc{{\buildrel {d}\over \longrightarrow}}
\def\defn{\skb\fl Definition\rm. }
\def\dens{\text{dens}}
\def\densC{\dens(\CC)}
\def\Dl{\Delta}
\def\dl{\delta}
\def\dnar{\downarrow}
\def\dpo{d_{P,1}}
\def\dpno{d_{P_n,1}}
\def\dpt{d_{P,2}}
\def\EE{{\Bbb E} }
\def\eee{\ =\ }
\def\eeq{\ \equiv \ }
\def\endp{\vfill\break}
\def\Eng{English transl.:}
\def\eps{\varepsilon}
\def\FF{{\cal F} }
\def\GG{{\cal G} }
\def\gee{\ \ge \ }
\def\goin{\to \infty}
\def\go0{\to 0}
\def\grad{\triangledown}
\def\fl{\smallskip}
%\def\fl{\flushpar} 
\def\HH{{\cal H} }
\def\inv{^{-1}}
\def\JJ{{\cal J} }
\def\KK{{\cal K} }
\def\la{\langle}
\def\li{< \infty}
\def\linF{\ell\upin(\FF)\ }
\def\lm{\lambda}
\def\Lm{\Lambda}
\def\lee{\ \le \ }
\def\leftitem#1{\item{\hbox to\parindent{\enspace#1\hfill}}}
\def\LL{{\cal L} }
\def\Lt{L^2(P)}
\def\Lto{L^2_0(P)}
\def\mc{m^{\CC }(}
\def\mcn{m^{\CC}(n)}
\def\mdsk{\medskip}
\def\mm{\vskip 1mm}
\def\MM{{\cal M} }
\def\nF{\|_{\FF}}
\def\NN{{\cal N} }
\def\normf{\|\cdot\|_{\cal F}}
\def\omg{\omega}
\def\Omg{\Omega}
\def\Omgap{(\Omg,\AA,{\rm Pr})\ }
\def\Omgsp{(\Omg, \Sigma ,{\rm Pr})\ }
\def\Omgspb{(\hat \Omg, \hat \Sigma ,\hat Pr)\ }
\def\Omgspr{(\Omg_{\eps }, \Sigma_{\eps } ,Pr_{\eps })\ }
\def\Omgspp{(\Omg_{\nu }, \Sigma_{\nu } , Pr_{\nu })\ }
\def\OO{{\bf O}}
\def\pard{\partial}
\def\pf{\hfill\break\bf Proof. \rm}
\def\pl{\ + \ }
\def\PP{{\cal P} }
\def\pr{probability}
\def\prm{^{\prime}}
\def\prc{{\buildrel {p}\over \longrightarrow}}
\def\prloc{{\buildrel {p,loc}\over \longrightarrow}}  
\def\prbloc{{\buildrel {{p, bloc}}\over \longrightarrow}}  
\def\qed{\hfill\break\rightline{$\bbox$}}
\def\QQ{{\cal Q}}
\def\ra{\rangle} 
\def\rbar{\overline{\Bbb R}}
\def\refs{\mdsk\cntr {REFERENCES}\mdsk}
\def\RR{{\Bbb R }}
\def\rtar{\Rightarrow}
\def\Ru{(in Russian)\ }
\def\sap{(S,\AA ,P)}
\def\soc{S(\CC )}
\def\setm{\setminus}
\def\sg{\sigma}
\def\sga{$\sigma$-algebra }
\def\sgal{$\sigma$-algebra}
\def\sg2{\sigma^2}
\def\sinph{\sin\phi}
\def\sinth{\sin\theta}
\def\skb{\medskip\fl\bf}
\def\sqt{^{1/2}}
\def\Sp{{\cal SP}(\RR^d)}
\def\SS{{\cal S} }
\def\SSSi{\smallint^{\infty}}
\def\SSOI{\smallint^1_0}
\def\SSS{\smallint}
\def\SSSW{\smallint^{\infty}_{-\infty}}
\def\tens{\otimes}
\def\TVMS{Teoria verojatnostej i matemati\v ceskaia statistika }
\def\TPA{\it Theor. Probability Appl. \bf}
\def\TPMS{Probability Theory and Mathematical Statistics, American
Mathematical Society} 
\def\tpr{\text{Pr}}
\def\TT{{\cal T} }
\def\subin{\_{\infty}}
\def\sumi{\sum^{\infty}}
\def\UMZ{Ukrainskij matemati\v ceskij \v zurnal}
\def\upar{\uparrow}
\def\upin{^{\infty}}
\def\VV{{\cal V}} 
\def\vc{Vapnik-\v Cervonenkis\ }
\def\wc{{\buildrel {w}\over \longrightarrow}}
\def\wloc{{\buildrel {w,loc}\over \longrightarrow}}  
\def\wbloc{{\buildrel {w, bloc }\over \longrightarrow}} 
\def\WW{{\cal W} } 
\def\XX{{\bf X} }
\def\xa{(\XX,\AA )\ }
\def\xap{(\XX,\AA,P)\ }
\def\xy{\{x,y\}}
\def\ZW{\it Z. Wahrscheinlichkeitsth. verw. Geb. \bf}
\def\ZZ{{\cal Z} }
\def\__{_{\infty}}
%\medskipamount=6pt plus 2pt minus 2pt










